VeriStruct: AI-assisted Automated Verification of Data-Structure Modules in Verus

We introduce VeriStruct, a novel framework that extends AI-assisted automated verification from single functions to more complex data structure modules in Verus. VeriStruct employs a planner module to orchestrate the systematic generation of abstractions, type invariants, specifications, and proof code. To address the challenge that LLMs often misunderstand Verus' annotation syntax and verification-specific semantics, VeriStruct embeds syntax guidance within prompts and includes a repair stage to automatically correct annotation errors. In an evaluation on eleven Rust data structure modules, VeriStruct succeeds on ten of the eleven, successfully verifying 128 out of 129 functions (99.2%) in total. These results represent an important step toward the goal of automatic AI-assisted formal verification.

==> macro.tex <==
% -----------------------------------------------------------------------------
% Draft toggle for notes and callouts
% Usage:
%   - Default: drafttrue (notes enabled)
%   - To disable in camera-ready: add `\draftfalse` BEFORE `\input{macro}`
% -----------------------------------------------------------------------------
\newif\ifdraft
\drafttrue


\ifdraft
  \RequirePackage{todonotes}
\else
  \RequirePackage[disable]{todonotes}
\fi

% TODOS (margin width can be tuned per template)
%\setlength{\marginparwidth}{1.5cm}

% Author comments and callouts
\ifdraft
  \newcommand{\cmscomment}[1]{\todo[color=blue!10,size=\small,fancyline,author=CMS]{#1}\xspace}
  \newcommand{\cmscommentinline}[1]{\todo[inline,color=blue!10,author=CMS]{#1}\xspace}
  \newcommand{\atcms}{\colorbox{blue!10}{\textit{@CMS}}}
  \newcommand{\yican}[1]{\todo[color=red!10,size=\small,fancyline,author=Yican]{#1}\xspace}
  \newcommand{\atyican}{\colorbox{red!10}{\textit{@Yican}}}
  \newcommand{\yxcomment}[1]{\todo[color=magenta!10,size=\small,fancyline,author=Yingfei]{#1}\xspace}
  \newcommand{\atxyf}{\colorbox{magenta!10}{\textit{@Yingfei}}}
  \newcommand{\ruyicomment}[1]{\todo[color=blue!10,size=\small,fancyline,author=Ruyi]{#1}\xspace}
  \newcommand{\atruyi}{\colorbox{blue!10}{\textit{@Ruyi}}}
\else
  \newcommand{\cmscomment}[1]{}
  \newcommand{\cmscommentinline}[1]{}
  \newcommand{\atcms}{}
  \newcommand{\yican}[1]{}
  \newcommand{\atyican}{}
  \newcommand{\yxcomment}[1]{}
  \newcommand{\atxyf}{}
  \newcommand{\ruyicomment}[1]{}
  \newcommand{\atruyi}{}
\fi


%% You could instead use the 'disable' option of todonotes
% \renewcommand{\cmscomment}[1]{}
% \renewcommand{\cmscommentinline}[1]{}
% \renewcommand{\atcms}{}
% \renewcommand{\yican}[1]{}
% \renewcommand{\atyican}{}
% \renewcommand{\yxcomment}[1]{}
% \renewcommand{\atxyf}{}
% \renewcommand{\ruyicomment}[1]{}
% \renewcommand{\atruyi}{}

%\newcommand{\ruyicomment}[1]{\textcolor{blue}{\textit{Ruyi:} #1}}

\newcommand{\eeq}{~{}={}~}
\newcommand{\ar}{\mathsf{ar}}
\newcommand{\kwtick}{\mathtt{pre}}
\newcommand{\kwinvoke}{\mathtt{invoke}}
\newcommand{\kwsample}{\mathtt{sample}}
\newcommand{\kwin}{\mathtt{in}}
\newcommand{\kwwith}{\bigoplus}
\newcommand{\com}{\mathsf{comm}}
\newcommand{\expr}{\mathsf{size}}
\newcommand{\pp}{\mathsf{expr}}
%\renewcommand{\skip}{\mathtt{skip}}
\newcommand{\dist}{\mathsf{dist}}
\newcommand{\etf}{\mathsf{Tf}}
\newcommand{\hm}{\mathsf{Hm}^{\mathsf{ub}}}
\newcommand{\emp}{\mathsf{emp}}
\newcommand{\body}{\mathsf{body}}
\newcommand{\rbody}{\mathsf{call}}
%\newcommand{\sem}[1]{\llbracket{#1}\rrbracket}
\newcommand{\sem}[1]{#1}
\newcommand{\pspace}{\mathrm{\Omega}}
\newcommand{\probspace}{(\pspace,\mathcal F,\Pr)}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\ex}{\mathsf{Ex}}
\newcommand{\prrlang}{{\sl LRec}}

\newcommand{\coef}{c}
\newcommand{\spolya}{p}
\newcommand{\sloga}{q}
\newcommand{\spolyn}{u}
\newcommand{\slogn}{v}
\newcommand{\coeff}{\coef_f}
\newcommand{\coeft}{\coef_t}
\newcommand{\logfa}{\sloga_{f}}
\newcommand{\logfn}{\slogn_{f}}
\newcommand{\polyfa}{\spolya_{f}}
\newcommand{\polyfn}{\spolyn_{f}}
\newcommand{\logta}{\sloga_{t}}
\newcommand{\logtn}{\slogn_{t}}
\newcommand{\polyta}{\spolya_{t}}
\newcommand{\polytn}{\spolyn_{t}}

\newcommand{\signature}{\theta}
\newcommand{\vardomain}{V}


\newcommand{\varmap}{\alpha}
\newcommand{\prog}{R}
\newcommand{\cont}{\mathbf{K}}
\newcommand{\cost}{C}
\newcommand{\conf}{\mu}

\newcommand{\seq}{\com_1;\com_2}
\newcommand{\invoke}{\kwinvoke\ p(\expr)}
\newcommand{\with}{\kwwith_{i=1}^k c_i\!:\!\com_i}
\newcommand{\sample}{\kwsample\ v\leftarrow\dist\ \kwin\ \{\body\}}
\newcommand{\tick}{\kwtick(\expr)}
\newcommand{\transprob}{\mathbf{P}}

\renewcommand{\paragraph}[1]{\smallskip\noindent{\textit{{#1.}}}}

%\newcommand{\todo}[1]{{\color{red} \it \{TODO: {#1}\}}}

\newcommand{\Nset}{\mathbb N}
\newcommand{\Zset}{\mathbb Z}
\newcommand{\Rset}{\mathbb R}
\newcommand{\Cset}{\mathbb C}
\newcommand{\proc}{\mbox{\sl proc}}
\newcommand{\fsdpd}{FSDPD}
\newcommand{\algexp}{\textsc{ExpSyn}}
\newcommand{\algpoly}{\textsc{PolySyn}}

\newcommand{\uniform}[1]{\textsc{Uniform}(#1)}
\newcommand{\muniform}[1]{\textsc{MUniform}(#1)}
\newcommand{\fbound}{\theta}

\newcommand{\pd}{\eta}
\newcommand{\condexpv}[2]{\expv\left[#1\ |\ #2\right]}
\newcommand{\dtsp}{\Gamma}

%%old macros from our previous submission
%\newcommand{\stack}{\mathcal S}
\newcommand{\coststack}{\mbox{\sl S}}
\newcommand{\eqtot}{m}
\newcommand{\recnum}{S}
\newcommand{\probm}{\Pr}
\newcommand{\sysnum}{O}
\newcommand{\fset}{\mathbb T}
\newcommand{\nset}{\mathbb N}
%\newcommand{\transf}{\mathcal P}
\newcommand{\transf}{f}
%\newcommand{\stacktrans}{\mathcal A}
\newcommand{\prev}{\mathcal O}
\newcommand{\lef}{{\le}_{\fspace}}
\newcommand{\sprr}{\Delta}
%\newcommand{\sprr}{\mathsf R}
\newcommand{\leinf}{{\le}_{\infspace}}
\newcommand{\botf}{{\bot}_{\fspace}}
\newcommand{\botinf}{{\bot}_{\infspace}}
\newcommand{\epxv}{\mathbb E}
\newcommand{\expv}{\epxv}
\newcommand{\tstack}{\mathcal A}
\newcommand{\cstack}{\mathcal Q}
%\renewcommand{\time}{T}
%\newcommand{\martingale}{\mathcal M}
\newcommand{\martingale}{\Psi}
\newcommand{\nxt}[1]{\mbox{\sl next}_{#1}}
\newcommand{\rtop}{\widehat{r}}
\newcommand{\ntop}{\widehat{n}}
\newcommand{\btop}{\widehat{\beta}}
\newcommand{\sktop}{\widehat{\sigma}}
\newcommand{\REC}{\mbox{\sl Rec}}
\newcommand{\BINOM}{\mbox{\sl Binom}}
\newcommand{\task}[1]{\textsc{#1}}
% Put your macros here
\newcommand{\livia}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\hf}[1]{{#1}}

 %for qedT mark compatible within displaymath
\def\triangleforqed{\hbox{$\lhd$}}
\makeatletter
\DeclareRobustCommand{\qedT}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\triangleforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\triangleforqed}%
	\fi
}
\makeatother

